Towards Robust EEG Decoding Based on Riemannian Self-Attention

Brain-Computer Interface (BCI) based on electroencephalography (EEG) enables direct interaction between the brain and external environments and has significant applications in assistive technologies, medical rehabilitation, and entertainment. Recently, EEG decoding methods based on Symmetric Positive Definite (SPD) learning have demonstrated superior performance. However, these methods typically employ basic network architectures and do not explicitly capture local relationships between EEG signals. This limitation is problematic for EEG signals due to their inherently low Signal-to-Noise Ratio (SNR). Moreover, most existing Riemannian manifold-based methods are restricted to specific metrics. The most widely used is the Affine-Invariant Metric (AIM). However, it has a quadratic dependency on the SPD matrices and cannot handle ill-conditioned SPD matrices, which hinders the effectiveness of networks. In contrast, the Bures-Wasserstein Metric (BWM) exhibits linear dependence on SPD matrices and demonstrates superior performance for ill conditioning. To overcome these challenges, we propose a Riemannian self-attention network based on the BWM. Additionally, the recently introduced power-deformed generalized Bures-Wasserstein metric reveals a nonlinear relationship between SPD matrices and matrix power deformation. This metric provides a more nuanced representation of the geometric structure of the SPD manifold. Consequently, we extend our model to a learnable version. For simplicity, we refer to it as GBWAtt. Experimental results on three EEG benchmarking datasets validate the robustness and effectiveness of our proposed method. The code is available at https://github.com/jissc/GBWAtt.

==> Section/2_related_work.tex <==
\section{Related work}
\label{sec:related work}

\subsection{Neural Networks for EEG}
Due to the superior feature extraction ability of deep learning, numerous end-to-end models have been proposed for electroencephalography (EEG) signal decoding~\cite{an2023dual}. To name a few, Santamaria et al.~\cite{santamaria2020eeg} introduced EEGInception, a novel ConvNets architecture based on the initial temporal network structure, which enables efficient and accurate classification of MI signals. Similarly, Zhang et al.~\cite{zhang2024convolutional} developed the Convolutional Dynamic Convergence Difference Neural Network (ConvDCDNN), achieving high accuracy of EEG signal classification with minimal human intervention.
FACT-Net~\cite{ke2024fact} enhances spectral feature representation by incorporating a frequency adapter module and employs a temporal-periodicity inception module to capture long-range temporal dependencies. Inspired by the brain’s cognitive mechanisms, Li et al.~\cite{li2024efficient} proposed a graph learning framework based on GCN to improve the performance of EEG-based emotion recognition. Although these methods have made significant progress in EEG signal decoding, they often fail to consider the inherent non-Euclidean geometric properties of EEG data. To address this issue, Suh et al.~\cite{suh2021riemannian} employed SPDNet to extract statistical features from EEG signals and introduced a separate-to-learn strategy. Pan et al.~\cite{pan2022matt} introduced MAtt, an SPD attention network leveraging the LEM to represent EEG signals as SPD matrices. Similarly, Wang et al.~\cite{gdlnet} proposed a novel Grassmannian Attention Network, which models channel features as Grassmann subspaces and implements self-attention mechanisms within the manifold space.



\subsection{Riemannian Networks for SPD Matrices}
Inspired by the superior feature extraction capability of ConvNets, Huang et al.~\cite{spdnet} proposed an end-to-end Riemannian neural network. Differently, this network is specifically designed to process structured data, enabling nonlinear, end-to-end learning on SPD matrices.  On this basis, Nguyen et al.~\cite{hgrnet} designed two aggregation subnetworks in the context of Gaussian embedded Riemannian manifolds for effectively encoding and learning spatial and temporal correlations. Zhang et al.~\cite{dmtnet} recognized the importance of local structural information for learning discriminative representations and introduced a 2D convolutional layer operating on SPD features, with convolution kernel matrix constrained to be SPD. Considering that this method does not respect the geometric structure of the data, Chakraborty et al.~\cite{manifoldnet} further proposed to simulate Euclidean convolution by calculating the weighted Fréchet mean over manifold-valued data grid, where each grid element corresponds to an SPD matrix, achieving better preservation of manifold properties. However, this approach does not explicitly capture the statistics within individual grid elements. Chen et al.~\cite{msnet} adhered more rigorously to the principles of Riemannian geometry by leveraging the category theory to abstract local structures on the SPD manifold, ultimately developing a a multi-scale network for capturing local geometric features.  Moreover, to enhance the applicability of Riemannian networks in visual tasks with limited training data, Wang et al.~\cite{symnet} developed a lightweight Riemannian network for SPD matrix nonlinear learning. This network employs a shallow optimization strategy for parameter learning, thereby improving computational efficiency while maintaining high classification accuracy.
